GraphMLP: A Graph MLP-Like Architecture for 3D Human Pose Estimation

Modern multi-layer perceptron (MLP) models have shown competitive results in learning visual representations without self-attention. However, existing MLP models are not good at capturing local details and lack prior knowledge of human body configurations, which limits their modeling power for skeletal representation learning. To address these issues, we propose a simple yet effective graph-reinforced MLP-Like architecture, named GraphMLP, that combines MLPs and graph convolutional networks (GCNs) in a global-local-graphical unified architecture for 3D human pose estimation. GraphMLP incorporates the graph structure of human bodies into an MLP model to meet the domain-specific demand of the 3D human pose, while allowing for both local and global spatial interactions. Furthermore, we propose to flexibly and efficiently extend the GraphMLP to the video domain and show that complex temporal dynamics can be effectively modeled in a simple way with negligible computational cost gains in the sequence length. To the best of our knowledge, this is the first MLP-Like architecture for 3D human pose estimation in a single frame and a video sequence. Extensive experiments show that the proposed GraphMLP achieves state-of-the-art performance on two datasets, i.e., Human3.6M and MPI-INF-3DHP. Code and models are available at https://github.com/Vegetebird/GraphMLP.

==> arxiv <==
\begin{thebibliography}{61}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[cod()]{code_baeline}
{Code for A Simple Yet Effective Baseline for {3D} Human Pose Estimation.}
\newblock \url{https://github.com/weigq/3d_pose_baseline_pytorch/}.

\bibitem[Ba et~al.(2016)Ba, Kiros, and Hinton]{ba2016layer}
Jimmy~Lei Ba, Jamie~Ryan Kiros, and Geoffrey~E Hinton.
\newblock Layer normalization.
\newblock \emph{arXiv preprint arXiv:1607.06450}, 2016.

\bibitem[Cai et~al.(2019)Cai, Ge, Liu, Cai, Cham, Yuan, and Thalmann]{stgcn}
Yujun Cai, Liuhao Ge, Jun Liu, Jianfei Cai, Tat-Jen Cham, Junsong Yuan, and
  Nadia~Magnenat Thalmann.
\newblock Exploiting spatial-temporal relationships for {3D} pose estimation
  via graph convolutional networks.
\newblock In \emph{ICCV}, pages 2272--2281, 2019.

\bibitem[Carion et~al.(2020)Carion, Massa, Synnaeve, Usunier, Kirillov, and
  Zagoruyko]{dert}
Nicolas Carion, Francisco Massa, Gabriel Synnaeve, Nicolas Usunier, Alexander
  Kirillov, and Sergey Zagoruyko.
\newblock End-to-end object detection with transformers.
\newblock In \emph{ECCV}, pages 213--229, 2020.

\bibitem[Chen et~al.(2023)Chen, He, Xiang, Cheng, Liu, Liu, Luo, Geng, and
  Xie]{chen2023hdformer}
Hanyuan Chen, Jun-Yan He, Wangmeng Xiang, Zhi-Qi Cheng, Wei Liu, Hanbing Liu,
  Bin Luo, Yifeng Geng, and Xuansong Xie.
\newblock {HDF}ormer: High-order directed transformer for {3D} human pose
  estimation.
\newblock In \emph{IJCAI}, pages 581--589, 2023.

\bibitem[Chen et~al.(2022)Chen, Xie, GE, Chen, Liang, and
  Luo]{chen2022cyclemlp}
Shoufa Chen, Enze Xie, Chongjian GE, Runjian Chen, Ding Liang, and Ping Luo.
\newblock Cycle{MLP}: A {MLP}-like architecture for dense prediction.
\newblock In \emph{ICLR}, 2022.

\bibitem[Chen et~al.(2021)Chen, Fang, Shen, Zhu, Chen, and
  Luo]{chen2021anatomy}
Tianlang Chen, Chen Fang, Xiaohui Shen, Yiheng Zhu, Zhili Chen, and Jiebo Luo.
\newblock Anatomy-aware {3D} human pose estimation with bone-based pose
  decomposition.
\newblock \emph{IEEE TCSVT}, 32\penalty0 (1):\penalty0 198--209, 2021.

\bibitem[Chen et~al.(2018)Chen, Wang, Peng, Zhang, Yu, and
  Sun]{chen2018cascaded}
Yilun Chen, Zhicheng Wang, Yuxiang Peng, Zhiqiang Zhang, Gang Yu, and Jian Sun.
\newblock Cascaded pyramid network for multi-person pose estimation.
\newblock In \emph{CVPR}, pages 7103--7112, 2018.

\bibitem[Ci et~al.(2019)Ci, Wang, Ma, and Wang]{ci2019optimizing}
Hai Ci, Chunyu Wang, Xiaoxuan Ma, and Yizhou Wang.
\newblock Optimizing network structure for {3D} human pose estimation.
\newblock In \emph{ICCV}, pages 2262--2271, 2019.

\bibitem[Dosovitskiy et~al.(2021)Dosovitskiy, Beyer, Kolesnikov, Weissenborn,
  Zhai, Unterthiner, Dehghani, Minderer, Heigold, Gelly, Uszkoreit, and
  Houlsby]{vit}
Alexey Dosovitskiy, Lucas Beyer, Alexander Kolesnikov, Dirk Weissenborn,
  Xiaohua Zhai, Thomas Unterthiner, Mostafa Dehghani, Matthias Minderer, Georg
  Heigold, Sylvain Gelly, Jakob Uszkoreit, and Neil Houlsby.
\newblock An image is worth 16x16 words: Transformers for image recognition at
  scale.
\newblock In \emph{ICLR}, 2021.

\bibitem[Gower(1975)]{gower1975generalized}
John~C Gower.
\newblock Generalized procrustes analysis.
\newblock \emph{Psychometrika}, 40\penalty0 (1):\penalty0 33--51, 1975.

\bibitem[Han et~al.(2022)Han, Yu, Gao, Sang, and Yang]{han2022single}
Chuchu Han, Xin Yu, Changxin Gao, Nong Sang, and Yi Yang.
\newblock Single image based {3D} human pose estimation via uncertainty
  learning.
\newblock \emph{PR}, 132:\penalty0 108934, 2022.

\bibitem[Hassan and Hamza(2023)]{hassan2023regular}
Md~Tanvir Hassan and A~Ben Hamza.
\newblock Regular splitting graph network for {3D} human pose estimation.
\newblock \emph{IEEE TIP}, 2023.

\bibitem[Hendrycks and Gimpel(2016)]{hendrycks2016gaussian}
Dan Hendrycks and Kevin Gimpel.
\newblock Gaussian error linear units ({GELU}s).
\newblock \emph{arXiv preprint arXiv:1606.08415}, 2016.

\bibitem[Hua et~al.(2022)Hua, Liu, Li, Zhang, Ding, and Xu]{hua2022weakly}
Guoliang Hua, Hong Liu, Wenhao Li, Qian Zhang, Runwei Ding, and Xin Xu.
\newblock Weakly-supervised {3D} human pose estimation with cross-view
  {U}-shaped graph convolutional network.
\newblock \emph{IEEE TMM}, 25:\penalty0 1832--1843, 2022.

\bibitem[Ionescu et~al.(2013)Ionescu, Papava, Olaru, and
  Sminchisescu]{ionescu2013human3}
Catalin Ionescu, Dragos Papava, Vlad Olaru, and Cristian Sminchisescu.
\newblock Human3.6{M}: Large scale datasets and predictive methods for {3D}
  human sensing in natural environments.
\newblock \emph{IEEE TPAMI}, 36\penalty0 (7):\penalty0 1325--1339, 2013.

\bibitem[Kim et~al.(2023)Kim, Lee, Nam, Jin, Kang, Yang, and
  Lee]{kim2023mhcanonnet}
Hyun-Woo Kim, Gun-Hee Lee, Woo-Jeoung Nam, Kyung-Min Jin, Tae-Kyung Kang,
  Geon-Jun Yang, and Seong-Whan Lee.
\newblock {MHC}anonnet: Multi-hypothesis canonical lifting network for
  self-supervised {3D} human pose estimation in the wild video.
\newblock \emph{PR}, page 109908, 2023.

\bibitem[Kipf and Welling(2016)]{kipf2016semi}
Thomas~N Kipf and Max Welling.
\newblock Semi-supervised classification with graph convolutional networks.
\newblock \emph{arXiv preprint arXiv:1609.02907}, 2016.

\bibitem[Li et~al.(2023{\natexlab{a}})Li, Shi, Dai, Zheng, Wang, Sun, Guo, Li,
  Zou, and Xiong]{li2023pose}
Han Li, Bowen Shi, Wenrui Dai, Hongwei Zheng, Botao Wang, Yu Sun, Min Guo,
  Chenglin Li, Junni Zou, and Hongkai Xiong.
\newblock Pose-oriented transformer with uncertainty-guided refinement for
  {2D}-to-{3D} human pose estimation.
\newblock In \emph{AAAI}, 2023{\natexlab{a}}.

\bibitem[Li et~al.(2023{\natexlab{b}})Li, Xiang, He, Cheng, Luo, Geng, and
  Xie]{li2023refined}
Hanbing Li, Wangmeng Xiang, Jun-Yan He, Zhi-Qi Cheng, Bin Luo, Yifeng Geng, and
  Xuansong Xie.
\newblock Refined temporal pyramidal compression-and-amplification transformer
  for {3D} human pose estimation.
\newblock \emph{arXiv preprint arXiv:2309.01365}, 2023{\natexlab{b}}.

\bibitem[Li et~al.(2018)Li, Han, and Wu]{li2018deeper}
Qimai Li, Zhichao Han, and Xiao-Ming Wu.
\newblock Deeper insights into graph convolutional networks for semi-supervised
  learning.
\newblock In \emph{AAAI}, 2018.

\bibitem[Li and Chan(2014)]{li20143d}
Sijin Li and Antoni~B Chan.
\newblock {3D} human pose estimation from monocular images with deep
  convolutional neural network.
\newblock In \emph{ACCV}, pages 332--347, 2014.

\bibitem[Li et~al.(2022{\natexlab{a}})Li, Liu, Ding, Liu, Wang, and
  Yang]{strided}
Wenhao Li, Hong Liu, Runwei Ding, Mengyuan Liu, Pichao Wang, and Wenming Yang.
\newblock Exploiting temporal contexts with strided transformer for {3D} human
  pose estimation.
\newblock \emph{IEEE TMM}, 25:\penalty0 1282--1293, 2022{\natexlab{a}}.

\bibitem[Li et~al.(2022{\natexlab{b}})Li, Liu, Tang, Wang, and
  Van~Gool]{mhformer}
Wenhao Li, Hong Liu, Hao Tang, Pichao Wang, and Luc Van~Gool.
\newblock {MHF}ormer: Multi-hypothesis transformer for {3D} human pose
  estimation.
\newblock In \emph{CVPR}, pages 13147--13156, 2022{\natexlab{b}}.

\bibitem[Li et~al.(2023{\natexlab{c}})Li, Liu, Tang, and Wang]{li2023multi}
Wenhao Li, Hong Liu, Hao Tang, and Pichao Wang.
\newblock Multi-hypothesis representation learning for transformer-based {3D}
  human pose estimation.
\newblock \emph{PR}, 141:\penalty0 109631, 2023{\natexlab{c}}.

\bibitem[Li et~al.(2024)Li, Liu, Liu, Wang, Cai, and Sebe]{hot}
Wenhao Li, Mengyuan Liu, Hong Liu, Pichao Wang, Jialun Cai, and Nicu Sebe.
\newblock Hourglass tokenizer for efficient transformer-based {3D} human pose
  estimation.
\newblock In \emph{CVPR}, pages 604--613, 2024.

\bibitem[Lian et~al.(2022)Lian, Yu, Sun, and Gao]{lian2021mlp}
Dongze Lian, Zehao Yu, Xing Sun, and Shenghua Gao.
\newblock {AS-MLP}: An axial shifted {MLP} architecture for vision.
\newblock In \emph{ICLR}, 2022.

\bibitem[Lin et~al.(2021)Lin, Wang, and Liu]{meshgraphormer}
Kevin Lin, Lijuan Wang, and Zicheng Liu.
\newblock Mesh {G}raphormer.
\newblock In \emph{ICCV}, pages 12939--12948, 2021.

\bibitem[Liu et~al.(2021{\natexlab{a}})Liu, Dai, So, and Le]{liu2021pay}
Hanxiao Liu, Zihang Dai, David So, and Quoc~V Le.
\newblock Pay attention to {MLP}s.
\newblock \emph{NeurIPS}, 34:\penalty0 9204--9215, 2021{\natexlab{a}}.

\bibitem[Liu et~al.(2023)Liu, He, Cheng, Xiang, Yang, Chai, Wang, Bao, Luo,
  Geng, et~al.]{liu2023posynda}
Hanbing Liu, Jun-Yan He, Zhi-Qi Cheng, Wangmeng Xiang, Qize Yang, Wenhao Chai,
  Gaoang Wang, Xu Bao, Bin Luo, Yifeng Geng, et~al.
\newblock Po{S}yn{DA}: Multi-hypothesis pose synthesis domain adaptation for
  robust {3D} human pose estimation.
\newblock In \emph{ACM MM}, pages 5542--5551, 2023.

\bibitem[Liu et~al.(2020{\natexlab{a}})Liu, Ding, Zou, Wang, and
  Tang]{liu2020comprehensive}
Kenkun Liu, Rongqi Ding, Zhiming Zou, Le Wang, and Wei Tang.
\newblock A comprehensive study of weight sharing in graph networks for {3D}
  human pose estimation.
\newblock In \emph{ECCV}, pages 318--334, 2020{\natexlab{a}}.

\bibitem[Liu et~al.(2020{\natexlab{b}})Liu, Shen, Wang, Chen, Cheung, and
  Asari]{liu2020attention}
Ruixu Liu, Ju Shen, He Wang, Chen Chen, Sen-ching Cheung, and Vijayan Asari.
\newblock Attention mechanism exploits temporal contexts: Real-time {3D} human
  pose reconstruction.
\newblock In \emph{CVPR}, pages 5064--5073, 2020{\natexlab{b}}.

\bibitem[Liu et~al.(2021{\natexlab{b}})Liu, Lin, Cao, Hu, Wei, Zhang, Lin, and
  Guo]{swin}
Ze Liu, Yutong Lin, Yue Cao, Han Hu, Yixuan Wei, Zheng Zhang, Stephen Lin, and
  Baining Guo.
\newblock Swin {T}ransformer: Hierarchical vision transformer using shifted
  windows.
\newblock In \emph{ICCV}, pages 10012--10022, 2021{\natexlab{b}}.

\bibitem[Martinez et~al.(2017)Martinez, Hossain, Romero, and
  Little]{simplebaseline}
Julieta Martinez, Rayat Hossain, Javier Romero, and James~J Little.
\newblock A simple yet effective baseline for {3D} human pose estimation.
\newblock In \emph{ICCV}, pages 2640--2649, 2017.

\bibitem[Mehraban et~al.(2024)Mehraban, Adeli, and Taati]{motionagformer}
Soroush Mehraban, Vida Adeli, and Babak Taati.
\newblock Motion{AGF}ormer: Enhancing {3D} human pose estimation with a
  transformer-gcnformer network.
\newblock In \emph{WACV}, pages 6920--6930, 2024.

\bibitem[Mehta et~al.(2017)Mehta, Rhodin, Casas, Fua, Sotnychenko, Xu, and
  Theobalt]{mehta2017monocular}
Dushyant Mehta, Helge Rhodin, Dan Casas, Pascal Fua, Oleksandr Sotnychenko,
  Weipeng Xu, and Christian Theobalt.
\newblock Monocular {3D} human pose estimation in the wild using improved {CNN}
  supervision.
\newblock In \emph{3DV}, pages 506--516, 2017.

\bibitem[Newell et~al.(2016)Newell, Yang, and Deng]{newell2016stacked}
Alejandro Newell, Kaiyu Yang, and Jia Deng.
\newblock Stacked hourglass networks for human pose estimation.
\newblock In \emph{ECCV}, pages 483--499, 2016.

\bibitem[Pavlakos et~al.(2017)Pavlakos, Zhou, Derpanis, and
  Daniilidis]{pavlakos2017coarse}
Georgios Pavlakos, Xiaowei Zhou, Konstantinos~G Derpanis, and Kostas
  Daniilidis.
\newblock Coarse-to-fine volumetric prediction for single-image {3D} human
  pose.
\newblock In \emph{CVPR}, pages 7025--7034, 2017.

\bibitem[Pavllo et~al.(2019)Pavllo, Feichtenhofer, Grangier, and
  Auli]{videopose}
Dario Pavllo, Christoph Feichtenhofer, David Grangier, and Michael Auli.
\newblock {3D} human pose estimation in video with temporal convolutions and
  semi-supervised training.
\newblock In \emph{CVPR}, pages 7753--7762, 2019.

\bibitem[Qiu et~al.(2023)Qiu, Qiu, Fu, and Fu]{qiu2023weakly}
Zhongwei Qiu, Kai Qiu, Jianlong Fu, and Dongmei Fu.
\newblock Weakly-supervised pre-training for {3D} human pose estimation via
  perspective knowledge.
\newblock \emph{PR}, 139:\penalty0 109497, 2023.

\bibitem[Ren et~al.(2021)Ren, Tang, and Sebe]{ren2021cascaded}
Bin Ren, Hao Tang, and Nicu Sebe.
\newblock Cascaded cross {MLP}-{M}ixer {GAN}s for cross-view image translation.
\newblock In \emph{BMVC}, 2021.

\bibitem[Shi et~al.(2022)Shi, Zhang, Tang, and Zhang]{shi2022polyp}
Jing-Hui Shi, Qing Zhang, Yu-Hao Tang, and Zhong-Qun Zhang.
\newblock Polyp-{M}ixer: An efficient context-aware {MLP}-based paradigm for
  polyp segmentation.
\newblock \emph{IEEE TCSVT}, 33\penalty0 (1):\penalty0 30--42, 2022.

\bibitem[Sun et~al.(2019)Sun, Xiao, Liu, and Wang]{hrnet}
Ke Sun, Bin Xiao, Dong Liu, and Jingdong Wang.
\newblock Deep high-resolution representation learning for human pose
  estimation.
\newblock In \emph{CVPR}, pages 5693--5703, 2019.

\bibitem[Tang et~al.(2023)Tang, Qiu, Hao, Hong, and Yao]{stcformer}
Zhenhua Tang, Zhaofan Qiu, Yanbin Hao, Richang Hong, and Ting Yao.
\newblock {3D} human pose estimation with spatio-temporal criss-cross
  attention.
\newblock In \emph{CVPR}, pages 4790--4799, 2023.

\bibitem[Tolstikhin et~al.(2021)Tolstikhin, Houlsby, Kolesnikov, Beyer, Zhai,
  Unterthiner, Yung, Steiner, Keysers, Uszkoreit, et~al.]{mlpmixer}
Ilya~O Tolstikhin, Neil Houlsby, Alexander Kolesnikov, Lucas Beyer, Xiaohua
  Zhai, Thomas Unterthiner, Jessica Yung, Andreas Steiner, Daniel Keysers,
  Jakob Uszkoreit, et~al.
\newblock {MLP}-{M}ixer: An all-{MLP} architecture for vision.
\newblock In \emph{NeurIPS}, pages 24261--24272, 2021.

\bibitem[Touvron et~al.(2021)Touvron, Bojanowski, Caron, Cord, El-Nouby, Grave,
  Izacard, Joulin, Synnaeve, Verbeek, et~al.]{touvron2021resmlp}
Hugo Touvron, Piotr Bojanowski, Mathilde Caron, Matthieu Cord, Alaaeldin
  El-Nouby, Edouard Grave, Gautier Izacard, Armand Joulin, Gabriel Synnaeve,
  Jakob Verbeek, et~al.
\newblock Res{MLP}: Feedforward networks for image classification with
  data-efficient training.
\newblock \emph{arXiv preprint arXiv:2105.03404}, 2021.

\bibitem[Vaswani et~al.(2017)Vaswani, Shazeer, Parmar, Uszkoreit, Jones, Gomez,
  Kaiser, and Polosukhin]{transformer}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones,
  Aidan~N Gomez, {\L}ukasz Kaiser, and Illia Polosukhin.
\newblock Attention is all you need.
\newblock In \emph{NeurIPS}, pages 5998--6008, 2017.

\bibitem[Wang et~al.(2014)Wang, Wang, Lin, Yuille, and Gao]{wang2014robust}
Chunyu Wang, Yizhou Wang, Zhouchen Lin, Alan~L Yuille, and Wen Gao.
\newblock Robust estimation of 3{D} human poses from a single image.
\newblock In \emph{CVPR}, pages 2361--2368, 2014.

\bibitem[Wang et~al.(2023)Wang, Wang, Deng, Wu, Wang, and Hao]{wang2023aa}
Qi Wang, JianJun Wang, Hongyu Deng, Xue Wu, Yazhou Wang, and Gefei Hao.
\newblock {AA}-trans: Core attention aggregating transformer with information
  entropy selector for fine-grained visual classification.
\newblock \emph{PR}, 140:\penalty0 109547, 2023.

\bibitem[Wei et~al.(2019)Wei, Lan, Zeng, and Chen]{wei2019view}
Guoqiang Wei, Cuiling Lan, Wenjun Zeng, and Zhibo Chen.
\newblock View invariant {3D} human pose estimation.
\newblock \emph{IEEE TCSVT}, 30\penalty0 (12):\penalty0 4601--4610, 2019.

\bibitem[Xu and Takano(2021)]{xu2021graph}
Tianhan Xu and Wataru Takano.
\newblock Graph stacked hourglass networks for {3D} human pose estimation.
\newblock In \emph{CVPR}, pages 16105--16114, 2021.

\bibitem[Zeng et~al.(2020)Zeng, Sun, Huang, Liu, Xu, and Lin]{zeng2020srnet}
Ailing Zeng, Xiao Sun, Fuyang Huang, Minhao Liu, Qiang Xu, and Stephen Lin.
\newblock {SRN}et: Improving generalization in {3D} human pose estimation with
  a split-and-recombine approach.
\newblock In \emph{ECCV}, pages 507--523, 2020.

\bibitem[Zeng et~al.(2021)Zeng, Sun, Yang, Zhao, Liu, and Xu]{zeng2021learning}
Ailing Zeng, Xiao Sun, Lei Yang, Nanxuan Zhao, Minhao Liu, and Qiang Xu.
\newblock Learning skeletal graph neural networks for hard {3D} pose
  estimation.
\newblock In \emph{ICCV}, pages 11436--11445, 2021.

\bibitem[Zhang et~al.(2022)Zhang, Tu, Yang, Chen, and Yuan]{mixste}
Jinlu Zhang, Zhigang Tu, Jianyu Yang, Yujin Chen, and Junsong Yuan.
\newblock Mix{STE}: Seq2seq mixed spatio-temporal encoder for {3D} human pose
  estimation in video.
\newblock In \emph{CVPR}, pages 13232--13242, 2022.

\bibitem[Zhang et~al.(2023)Zhang, Wang, Nie, Yao, Huang, and
  Tian]{zhang2023learning}
Shengping Zhang, Chenyang Wang, Liqiang Nie, Hongxun Yao, Qingming Huang, and
  Qi Tian.
\newblock Learning enriched hop-aware correlation for robust {3D} human pose
  estimation.
\newblock \emph{IJCV}, 131\penalty0 (6):\penalty0 1566--1583, 2023.

\bibitem[Zhao et~al.(2019)Zhao, Peng, Tian, Kapadia, and
  Metaxas]{zhao2019semantic}
Long Zhao, Xi Peng, Yu Tian, Mubbasir Kapadia, and Dimitris~N Metaxas.
\newblock Semantic graph convolutional networks for {3D} human pose regression.
\newblock In \emph{CVPR}, pages 3425--3435, 2019.

\bibitem[Zhao et~al.(2022{\natexlab{a}})Zhao, Wang, and
  Tian]{zhao2022graformer}
Weixi Zhao, Weiqiang Wang, and Yunjie Tian.
\newblock Gra{F}ormer: Graph-oriented transformer for {3D} pose estimation.
\newblock In \emph{CVPR}, pages 20438--20447, 2022{\natexlab{a}}.

\bibitem[Zhao et~al.(2022{\natexlab{b}})Zhao, Wu, Zhuang, Li, and
  Jia]{zhao2022tracking}
Zelin Zhao, Ze Wu, Yueqing Zhuang, Boxun Li, and Jiaya Jia.
\newblock Tracking objects as pixel-wise distributions.
\newblock In \emph{ECCV}, 2022{\natexlab{b}}.

\bibitem[Zheng et~al.(2021)Zheng, Zhu, Mendieta, Yang, Chen, and
  Ding]{poseformer}
Ce Zheng, Sijie Zhu, Matias Mendieta, Taojiannan Yang, Chen Chen, and Zhengming
  Ding.
\newblock {3D} human pose estimation with spatial and temporal transformers.
\newblock In \emph{ICCV}, pages 11656--11665, 2021.

\bibitem[Zhu et~al.(2021)Zhu, Su, Lu, Li, Wang, and Dai]{zhu2020deformable}
Xizhou Zhu, Weijie Su, Lewei Lu, Bin Li, Xiaogang Wang, and Jifeng Dai.
\newblock Deformable {DETR}: Deformable transformers for end-to-end object
  detection.
\newblock In \emph{ICLR}, 2021.

\bibitem[Zou and Tang(2021)]{zou2021modulated}
Zhiming Zou and Wei Tang.
\newblock Modulated graph convolutional network for {3D} human pose estimation.
\newblock In \emph{ICCV}, pages 11477--11487, 2021.

\end{thebibliography}

